VISAGE: Video Instance Segmentation with Appearance-Guided Enhancement

In recent years, online Video Instance Segmentation (VIS) methods have shown remarkable advancement with their powerful query-based detectors. Utilizing the output queries of the detector at the frame-level, these methods achieve high accuracy on challenging benchmarks. However, our observations demonstrate that these methods heavily rely on location information, which often causes incorrect associations between objects. This paper presents that a key axis of object matching in trackers is appearance information, which becomes greatly instructive under conditions where positional cues are insufficient for distinguishing their identities. Therefore, we suggest a simple yet powerful extension to object decoders that explicitly extract embeddings from backbone features and drive queries to capture the appearances of objects, which greatly enhances instance association accuracy. Furthermore, recognizing the limitations of existing benchmarks in fully evaluating appearance awareness, we have constructed a synthetic dataset to rigorously validate our method. By effectively resolving the over-reliance on location information, we achieve state-of-the-art results on YouTube-VIS 2019/2021 and Occluded VIS (OVIS). Code is available at https://github.com/KimHanjung/VISAGE.

==> fig/analysis_appearance.tex <==
% \begin{figure}[t]
%   \centering
%   \begin{minipage}{.5\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{fig_img/tsne_tworow.pdf}
%     \vspace{-4mm}
%     \caption{
%     \textbf{T-SNE visualization on the OVIS dataset.}
%     Each row representing three different videos. 
%     Each column corresponds to the type of query embedding utilized. 
%     Points plotted in the same color indicate the same instance across the dataset. Best viewed in color.
%     }
%     \vspace{-4mm}
%     \label{fig:tsne}
%   \end{minipage}%
%   \hfill
%   \begin{minipage}{.45\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{fig_img/pseudo.pdf}
%     \vspace{-5mm}
%     \caption{
%     \textbf{Visualization of the pseudo dataset.}
%     In \textit{track type} videos, instances move along random bezier curves.
%     On the other hand, the \textit{swap type} refers to a scenario where the positions of each instance are exchanged in the middle of the video. The colored dot above each instance represents the corresponding instance in the swapped frame.
%     }
%     \vspace{-2mm}
%     \label{fig:pseudo}
%   \end{minipage}
% \end{figure}


% \begin{figure}[t]
% \centering
% \includegraphics[width=0.7\linewidth]{fig_img/tsne_tworow.pdf}
% \caption{
% \textbf{T-SNE visualization on the OVIS dataset.}
% Each row representing three different videos. 
% Each column corresponds to the type of query embedding utilized. 
% Points plotted in the same color indicate the same instance across the dataset. Best viewed in color.
% }
% \label{fig:tsne}
% \end{figure}
% \begin{figure}[t]
% \centering
% \includegraphics[width=0.7\linewidth]{fig_img/pseudo.pdf}
% \caption{
% \textbf{Visualization of the pseudo dataset.}
% In \textit{track type} videos, instances move along random bezier curves.
% On the other hand, the \textit{swap type} refers to a scenario where the positions of each instance are exchanged in the middle of the video. The colored dot above each instance represents the corresponding instance in the swapped frame.
% }
% \label{fig:pseudo}
% \end{figure}

\begin{figure}[t!]
  \centering
  \begin{minipage}{\textwidth}
    \centering
    \includegraphics[width=0.8\linewidth]{fig_img/pseudo.pdf}
    \caption{
    \textbf{Visualization of the pseudo dataset.}
    In \textit{track type} videos, instances move along random bezier curves.
    On the other hand, the \textit{swap type} refers to a scenario where the positions of each instance are exchanged in the middle of the video. The colored dot above each instance represents the corresponding instance in the swapped frame.
    }
    \label{fig:pseudo}
  \end{minipage}
  \vspace{6mm}
  \begin{minipage}{\textwidth}
    \centering
    % \includegraphics[width=0.7\linewidth]{fig_img/tsne_tworow.pdf}
    % \caption{
    % \textbf{T-SNE visualization on the OVIS dataset.}
    % Each row representing three different videos. 
    % Each column corresponds to the type of query embedding utilized. 
    % Points plotted in the same color indicate the same instance across the dataset. Best viewed in color.
    % }
    % \label{fig:tsne}
    \captionof{table}{Comparisons on \textbf{Pseudo dataset}.}
    % \vspace{-2mm}
    \begin{tabular}{@{}c|l|c|ccccc@{}}
        \toprule
        \multicolumn{2}{l|}{Method}   & App           & AP        & AP$_{50}$     & AP$_{75}$     & AR$_{1}$      & AR$_{10}$ \\
        % & Method   & App           & AP        & AP$_{50}$     & AP$_{75}$     & AR$_{1}$      & AR$_{10}$ \\
        \midrule
        \midrule
        
        % \multicolumn{2}{l|}{IDOL~\cite{IDOL}}             & \multirow{4}{*}{track}
        %                                                                   & 57.9      & 76.3      & 62.9      & 62.9      & 65.9      \\
        \multirow{4}{*}{\rotatebox{90}{Track}}
        & GenVIS~\cite{GenVIS}      &                & 54.8      & 70.6      & 58.8      & 61.2      & 65.9   \\ 
        & CTVIS~\cite{CTVIS}        &                & 63.7      & 78.7      & 69.7      & 70.3      & 74.8   \\ 
        % \cmidrule{2-8}
        & \name{}                   &                & 65.2      & 80.9      & 71.3      & 70.2      & 75.2   \\ 
        & \name{}                   & \cmark         & \textbf{65.8}      & \textbf{81.1}          & \textbf{71.7}          & \textbf{70.8}          & \textbf{76.3}   \\ 
        \midrule
        % \multicolumn{2}{l|}{IDOL~\cite{IDOL}}             & \multirow{4}{*}{swap}
        %                                                                   & 42.8      & 64.8      & 44.1      & 50.5      & 53.4      \\
        \multirow{4}{*}{\rotatebox{90}{Swap}}
        & GenVIS~\cite{GenVIS}      &                & 41.8      & 59.7      & 44.0      & 50.8      & 57.0   \\ 
        & CTVIS~\cite{CTVIS}        &                & 53.1      & 71.7      & 56.9      & 61.7      & 65.7   \\ 
        % \cmidrule{2-8}
        & \name{}                   &                & 51.8      & 72.1      & 54.4      & 57.7      & 62.8   \\ 
        & \name{}                   & \cmark         & \textbf{63.0}      & \textbf{79.5}          & \textbf{69.3}          & \textbf{67.8}          & \textbf{73.5}   \\ 
        \bottomrule
    \end{tabular}
    \label{tab:pseudo}
  \end{minipage}%
\vspace{-7mm}
\end{figure}

==> fig/appearance_tsne.tex <==
\begin{figure}[t]

\begin{minipage}[c]{0.45\linewidth}
    \centering
    \captionof{table}{Ablation study on appearance weightage.}
    % \vspace{-2mm}
    \resizebox{\linewidth}{!}{
    % \begin{tabular}{@{}c|ccccc|ccccc@{}}
    %     \toprule
    %     \multirow{2}{*}{\shortstack{$\alpha$}} &   \multicolumn{5}{c|}{YouTube-VIS 2019} &   \multicolumn{5}{c}{OVIS}\\
    %                 & AP        & AP$_{50}$ & AP$_{75}$ & AR$_1$    & AR$_{10}$      & AP        & AP$_{50}$ & AP$_{75}$ & AR$_1$    & AR$_{10}$      \\
    %         \midrule
    %         \midrule
    %       0.00      & 53.4      & 76.8      & 58.7      & 49.8      & 61.2      
    %                 & 32.2      & 55.6      & 30.9      & 16.1      & 36.3      \\
    %       0.25      & 53.6      & 77.0      & 59.4      & 50.0      & 61.1      
    %                 & 34.5      & 59.2      & 32.5      & 16.7      & 38.8      \\
    %       0.50      & 54.5      & 77.2      & 60.3      & 50.9      & 61.7      
    %                 & 34.8      & 59.8      & 35.3      & 16.2      & 39.4      \\
    %       \rowcolor{gray!=25}
    %       0.75      & 55.1      & 78.1      & 50.6      & 51.0      & 62.3      
    %                 & 36.2      & 60.3      & 35.3      & 17.0      & 40.3      \\
    %       1.00      & 24.9      & 36.7      & 28.7      & 40.9      & 53.7      
    %                 & 11.4      & 22.7      & 10.2      & 10.3      & 24.9      \\
    %     \bottomrule
    % \end{tabular}}
    \begin{tabular}{@{}c|ccccc@{}}
        \toprule
        \multirow{2}{*}{\shortstack{$\alpha$}}  &   \multicolumn{5}{c}{OVIS}\\
                     & AP        & AP$_{50}$ & AP$_{75}$ & AR$_1$    & AR$_{10}$      \\
            \midrule
            \midrule
          0.00      & 32.2      & 55.6      & 30.9      & 16.1      & 36.3      \\
          0.25      & 34.5      & 59.2      & 32.5      & 16.7      & 38.8      \\
          0.50      & 34.8      & 59.8      & 35.3      & 16.2      & 39.4      \\
          \rowcolor{gray!=25}
          0.75      & 36.2      & 60.3      & 35.3      & 17.0      & 40.3      \\
          1.00      & 11.4      & 22.7      & 10.2      & 10.3      & 24.9      \\
        \bottomrule
    \end{tabular}}
    % \resizebox{\linewidth}{!}{
    % \begin{tikzpicture}
    %     \begin{axis}[
    %         title={\textbf{Analysis of Appearance Weight $\alpha$}},
    %         xlabel={$\alpha$},
    %         ylabel={AP},
    %         xmin=0, xmax=1,
    %         ymin=0, ymax=40,
    %         xtick={0,0.25,0.50,0.75,1},
    %         ytick={0,10,20,30,40,50,60},
    %         extra y ticks={36.2},
    %         extra y tick labels={36.2},
    %         extra y tick style={grid=major, grid style={dashed}},
    %         legend pos=north west,
    %         ymajorgrids=true,
    %         grid style=dashed,
    %         axis line style={draw=none}, % Removes the axis lines
    %         tick style={draw=none}, % Removes the ticks
    %     ]
        
    %     \addplot[
    %         color=CadetBlue,
    %         mark=square,
    %         line width=1.5pt,
    %         ]
    %         coordinates {
    %         (0.00,32.2) (0.25,34.5) (0.50,34.8) (0.75,36.2) (1.00,11.4)
    %         };

    %     % \addplot[
    %     %     color=Mahogany,
    %     %     mark=square,
    %     %     line width=1.5pt,
    %     %     ]
    %     %     coordinates {
    %     %     (0.00,53.4) (0.25,53.6) (0.50,54.5) (0.75,55.1) (1.00,24.9)
    %     %     };
        
    %     \end{axis}
    % \end{tikzpicture}}
    % \caption{\textbf{Analysis of Appearance Weight $\alpha$.} The plot demonstrates the relationship between different appearance weight $\alpha$ settings and their corresponding AP scores on the OVIS dataset.}
    % \label{fig:appearance}
\end{minipage}%
\hfill
\begin{minipage}[c]{0.5\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{fig_img/tsne_tworow_2.pdf}
    \caption{
    \textbf{T-SNE visualization on the OVIS dataset.}
    Each row representing three different videos. 
    Each column corresponds to the type of query embedding utilized. 
    Points plotted in the same color indicate the same instance across the dataset. Best viewed in color.
    }
    \label{fig:tsne}
\end{minipage}
\vspace{-3mm}
\end{figure}



==> fig/pseudo.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.7\linewidth]{fig_img/pseudo.pdf}
\caption{
\textbf{Visualization of the pseudo dataset.}
In \textit{track type} videos, instances move along random bezier curves.
On the other hand, the \textit{swap type} refers to a scenario where the positions of each instance are exchanged in the middle of the video. The colored dot above each instance represents the corresponding instance in the swapped frame.
}
\label{fig:pseudo}
\vspace{-2mm}
\end{figure}

==> fig/sup_teaser.tex <==
\begin{figure*}[t]
\begin{center}
   \includegraphics[width=\linewidth]{fig_img/sup_teaser.pdf}
\end{center}
\vspace{-6mm}
\caption{ 
\textbf{Additional qulitative results} present a side-by-side comparison of our method, \name{}, with previous methods~\cite{MinVIS, IDOL, GenVIS, DVIS, CTVIS} on various scenarios. 
Each row showcases the predicted results from different methods, with \name{} distinctly achieving accurate predictions. 
Consistency across evaluations is maintained by employing the same backbone and benchmark-trained weights for all methods, as illustrated in this collection of images.
}
\vspace{-2mm}
\label{fig:sup_teaser}
\end{figure*}

==> tab/ablation_efficiency.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}
{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}l|cc|ccc@{}}
\toprule
Method      & GFLOPs    & P\\
    \midrule
    \midrule

heuristic (w/o NMS)  & 52.7      & 75.3      & 57.6      & 49.3      & 61.6      \\
heuristic (w/ NMS)   & 54.4      & 77.9      & 59.0      & 49.9      & 62.8      \\
simple               & 54.5      & 77.2      & 60.3      & 50.9      & 61.7      \\
    \bottomrule
    \end{tabular}
} %< \resizebox
\vspace{-2mm}
\caption{
% 
Ablation study of the tracker type on YTVIS 2019 validation set.
% 
}
\vspace{-3mm}
\label{tab:ablation_efficiency}
\end{table}

==> tab/ablation_window_size.tex <==
\begin{table}
\centering

\resizebox{0.8\linewidth}{!}
{ %< auto-adjusts font size to fill line
\caption{
% 
Ablation study of the window size $W$.
% 
}
\begin{tabular}{@{}c|ccccc@{}}
\toprule
$W$                  & AP        & AP$_{50}$ & AP$_{75}$ & AR$_1$    & AR$_{10}$ \\
    \midrule
    \midrule

2  & 53.2      & 75.2      & 58.7      & 50.1      & 62.1      \\
3  & 54.6      & 76.8      & 60.3      & 50.3      & 62.7      \\
\rowcolor{gray!=25}
5  & 55.1      & 78.1      & 60.6      & 51.0      & 62.3      \\
10 & 54.0      & 76.4      & 59.9      & 50.2      & 61.6      \\
    \bottomrule
    \end{tabular}
} %< \resizebox
\vspace{-2mm}
% \vspace{-3mm}
\label{tab:ablation_window_size}
\vspace{-2mm}
\end{table}

==> tab/efficiency.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}
{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}l|ccc|ccc@{}}
\toprule
% Method            & FPS        & Params     & GFLOPs\\
\multirow{2}{*}{Method}          & \multicolumn{3}{c|}{Metric}  & \multirow{2}{*}{\shortstack{YTVIS\\2019}} & \multirow{2}{*}{\shortstack{YTVIS\\2021}} & \multirow{2}{*}{OVIS} \\
                     & FPS       & Params  & GFLOPs      &       &       \\
    \midrule
    \midrule

MinVIS~\cite{MinVIS} & 25.6      & 44      & 3031        & 47.4  & 44.2     & 25.0 \\
CTVIS~\cite{CTVIS}   & 13.2      & 44      & 3036        & 55.1  & 50.1     & 35.5 \\
VISAGE               & 23.3      & 45      & 3083        & 54.5  & 50.8     & 34.8 \\
    \bottomrule
    \end{tabular}
} %< \resizebox
\vspace{-2mm}
\caption{
% 
Computation Comparison on YTVIS 2019 validation set.
% 
}
\vspace{-3mm}
\label{tab:efficiency}
\end{table}

% \begin{table}
% \centering
% \resizebox{0.7\linewidth}{!}
% { %< auto-adjusts font size to fill line
% \begin{tabular}{@{}l|ccc|ccc@{}}
% \toprule
% % Method            & FPS        & Params     & GFLOPs\\
% \multirow{2}{*}{Method}                        & \multirow{2}{*}{\shortstack{YTVIS\\2019}} & \multirow{2}{*}{\shortstack{YTVIS\\2021}} & \multirow{2}{*}{OVIS} \\
% & & & \\
%     \midrule
%     \midrule

% MinVIS~\cite{MinVIS} & 25.6      & 44      & 3031  \\
% CTVIS~\cite{CTVIS}   & 13.2      & 44      & 3036  \\
% VISAGE               & 23.3      & 45      & 3083  \\
%     \bottomrule
%     \end{tabular}
% } %< \resizebox
% \vspace{-2mm}
% \caption{
% % 
% Computation Comparison on YTVIS 2019 validation set.
% % 
% }
% \vspace{-3mm}
% \label{tab:efficiency}
% \end{table}

==> tab/idol_module.tex <==
\begin{table*}
\centering
\resizebox{\linewidth}{!}
{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lc|l|cccccc|cccccc@{}}
\toprule
\multicolumn{2}{l|}{\multirow{2}{*}{Method}}                        & \multirow{2}{*}{Backbone} & \multicolumn{6}{c|}{YouTube-VIS 2019} & \multicolumn{6}{c}{YouTube-VIS 2021}\\
\multicolumn{2}{l|}{}                                               &          & AP        & $\Delta_{AP}$  & AP$_{50}$ & AP$_{75}$ & AR$_1$    & AR$_{10}$ & AP        & $\Delta_{AP}$  & AP$_{50}$ & AP$_{75}$ & AR$_1$    & AR$_{10}$ \\
    \midrule
    \midrule
    
    %%% R50
    \multicolumn{2}{l|}{IDOL~\cite{IDOL}}                         & ResNet-50  & 46.4      &                & 70.7      & 51.9      & 44.8      & 54.9   
                                                                               & 43.9      &                & 68.0      & 49.6      & 38.0      & 50.9  \\
    % \cmidrule{2-14}
    \multicolumn{2}{l|}{IDOL+Appearance}                          & ResNet-50  & 46.7      & \textcolor{red}{+0.3}  & 71.0      & 49.1      & 46.4      & 56.1   
                                                                               & 46.2      & \textcolor{red}{+2.3}  & 69.1      & 49.4      & 39.3      & 54.0  \\
    \bottomrule
    \end{tabular}
} %< \resizebox
\vspace{-2mm}
\caption{
% 
Comparisons on \textbf{YouTube-VIS 2019 and 2021 validation} sets.
% The results are firstly grouped into online and semi-online or offline settings, and then, light-weight (\emph{e.g.}, ResNet-50, MsgShifT) and powerful (\emph{e.g.}, Swin-L) backbone networks.
We group the results by online or not online methods, and then, lightweight (\emph{e.g.}, ResNet-50) or powerful (\emph{e.g.}, Swin-L) backbone networks.
For each group, we \textbf{bold} the best value in every metric.
% 
}
\vspace{-3mm}
\label{tab:ytvis2019_2021}
\end{table*}
